Efficient Sensor Placement from Regression with Sparse Gaussian Processes in Continuous and Discrete Spaces

The sensor placement problem is a common problem that arises when monitoring correlated phenomena, such as temperature, precipitation, and salinity. Existing approaches to this problem typically formulate it as the maximization of information metrics, such as mutual information~(MI), and use optimization methods such as greedy algorithms in discrete domains, and derivative-free optimization methods such as genetic algorithms in continuous domains. However, computing MI for sensor placement requires discretizing the environment, and its computation cost depends on the size of the discretized environment. These limitations restrict these approaches from scaling to large problems. We present a novel formulation to the SP problem based on variational approximation that can be optimized using gradient descent, allowing us to efficiently find solutions in continuous domains. We generalize our method to also handle discrete environments. Our experimental results on four real-world datasets demonstrate that our approach generates sensor placements consistently on par with or better than the prior state-of-the-art approaches in terms of both MI and reconstruction quality, all while being significantly faster. Our computationally efficient approach enables both large-scale sensor placement and fast robotic sensor placement for informative path planning algorithms.

==> transformations.tex <==
\subsection{Linear and Non-linear Transformations}
\label{sec:transformations}

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\linewidth]{figures/overview.pdf}
    \caption{An illustration of the sensor placement approach for sparse view CT scanning with fan beam projections. The expansion transformation maps each of the $m$ inducing points in the point parametrization to $p$ points in the FoV parametrization to approximate each sensor's FoV, and the aggregation transformation aggregates the covariances corresponding to the $mp$ points to model the sensor's integrated observations.}
    \label{fig:overview}
\end{figure*}

We now generalize our approach to handle sensors with non-point FoV and integrated observations. Although such sensor models have been attempted in prior work, our sensor placement approach's computational efficiency allows us to address significantly larger problems. As an illustrative example, we consider the problem of sensor placement for sparse view computed tomography (CT)~\cite{LongiRSMRSHK20}.

A third-generation fan beam CT scanner~\cite{Zeng17} projects X-ray beams that fan out at a fixed angle~(Figure~\ref{fig:overview}). On the opposite side of the projector, a sensor array captures data integrated along each beam and encoded by the received X-ray intensity. The projector and sensor array pair rotate around a circular area of interest, and the collected data is then used to reconstruct the underlying spatially resolved data. Being able to compute informative sensor placements efficiently is especially useful when the region of interest is a sub-region of the observation space (e.g., if we only need to scan a specific organ), as we will be able to optimize the sensor placements in real-time, thereby reducing the amount of harmful X-ray exposure to patients while also retaining reconstruction quality.

A key advantage of our sensor placement approach is that we can leverage all the proprieties of GPs and SGPs~\cite{RasmussenW05, SmithP05, Titsias09}. We detail two such properties and how they are used to address sensor placement for sensors with non-point FoV and integrated observations. 

The first property is that the inducing points of SGPs can be transformed with any non-linear function and still be optimized using gradient descent. We can use such transformations to approximate the FoV of a sensor with non-point FoV. We do this by parameterizing each inducing point of the SGP as a point on the edge of the circular observation space. To account for the information from each sensor's whole FoV (X-ray beams within the fan angle), we apply a transformation—the expansion transformation $T_\text{exp}$—to map each inducing point to a set of $p$ points that approximate the region within the corresponding sensor's FoV as follows: $\mathbf{X}_{mp} = T_\text{exp}(\mathbf{X}_{m})$. The expansion transformation is applied to the inducing points $\mathbf{X}_{m} \in \mathbb{R}^{m \times \Bar{d}}$ to get the FoV parametrized inducing points $\mathbf{X}_{mp} \in \mathbb{R}^{mp \times d}$ before computing any covariance matrix involving the inducing points. Thus, we can still calculate the gradients for the inducing points with the point parametrization. Here $\Bar{d}$ is the dimension of the inducing points with point parametrization, and $d$ is the dimension of the sensor placement environment $\mathcal{V}$.

The second property we utilize is that GPs are closed under linear transformations~\cite{RasmussenW05}. We can leverage the property to model sensors with integrated observations~\cite{LongiRSMRSHK20}, i.e., where the labels are modeled as $y_i = ||\mathbf{w}_i|| \int_0^1 f(\mathbf{w}_i t+\mathbf{z}_i)dt + \epsilon_i$, with $\mathbf{z}_i$ as the start point of a line along which the data is integrated, and $\mathbf{w}_i$ as the direction and length of the line. We do this with the aggregation transformation $T_\text{agg}$, which aggregates (with an averaging operation) the covariances corresponding to the $p$ points that approximate each sensor's FoV and reduces the size of the covariance matrix back to $m \times m$.

We first use the expansion transformation ($T_\text{exp}$) on the $m$ inducing points to map them from point  parametrization to a larger set of $mp$ points. Then we use the aggregation transformation $T_\text{agg}$ on the covariance matrices built using the $mp$ points. The covariances are used to compute $\mathbf{Q}_{nn}$, which is, in turn, used to compute the  SVGP's lower bound~(Equation~\ref{vfe}):

\begin{equation}
\begin{aligned}
\label{Q_nn}
\mathbf{Q}_{nn} &= \mathbf{K}_{n \times mp}T_\text{agg} (T_\text{agg}^\top \mathbf{K}_{mp \times mp}T_\text{agg})^{-1} T_\text{agg}^\top \mathbf{K}_{mp \times n}\,.
\end{aligned}
\end{equation}

Here $\mathbf{K}_{n \times mp}$ is the covariance between the $n$ training set inputs and the $mp$ inducing points. The aggregation transformation reduces the covariance matrices before inversion. The approach is illustrated in~\fgref{fig:overview}, and further details of how to define the transformations are presented in the appendix. Therefore, the inversion operation cost is reduced to $\mathcal{O}(m^3)$ from $\mathcal{O}(m^3p^3)$. Thus we reap the benefits of the compact point parametrization from the expansion transformation and the reduced computation cost from the aggregation transformation. We found that the aggregation transformation also stabilized the gradients while training the inducing points.
